Partially Constrained Group Variable Selection to Adjust for Complementary Unit Performance in American College Football

Given the importance of accurate team rankings in American college football (CFB) -- due to heavy title and playoff implications -- strides have been made to improve evaluation metrics across statistical categories, going from basic averages (e.g. points scored per game) to metrics that adjust for a team's strength of schedule, but one aspect that hasn't been emphasized is the complementary nature of American football. Despite the same team's offensive and defensive units typically consisting of separate player sets, some aspects of your team's defensive (offensive) performance may affect the complementary side: turnovers forced by your defense could lead to easier scoring chances for your offense, while your offense's ability to control the clock may help your defense. For 2009-2019 CFB seasons, we incorporate natural splines with group penalty approaches to identify the most consistently influential features of complementary football in a data-driven way, conducting partially constrained optimization in order to additionally guarantee the full adjustment for strength of schedule and homefield factor. We touch on the issues arising due to reverse-causal nature of certain within-game dynamics, discussing several potential remedies. Lastly, game outcome prediction performances are compared across several ranking adjustment approaches for method validation purposes.

==> Arxiv_Submission/10_Figures.tex <==

\newpage




\begin{figure}[H]
\begin{center}
 \includegraphics[scale=0.8]{Images/GROUP_LASSO_SELECTION_STABILITY_MATRIX.png}
\end{center}
\caption{%\textbf{A weighted proportion of times a natural cubic spline representing a particular complementary football statistic (rows) was selected across different group penalties and tuning parameter selection approaches.}
}
\label{fig: EfficiencyConsistencySelection}
\end{figure}

\newpage




\begin{figure}[H]
\begin{center}
 \includegraphics[scale=0.45]{Images/Pts_on_TO_and_Yds_on_YdsPPlay.png}
\end{center}
\caption{%\textbf{Non-linear effects of complementary statistics on respective response categories, controlling for strength of schedule and homefield factor. Left: Effect of non-scoring turnovers forced by your defense on points scored by your offense. Right: Effect of per-play yardage allowed by your defense on yards gained by your offense.} These particular effect graphics were obtained for a Navy versus Army match-up at a neutral site. Changing the match-up would only affect the intercepts, hence there's no loss of generality in depicting the nature of the effect.
}
\label{fig: NonLinearEffects_Graphs_Efficiency_Stats}
\end{figure}








==> Arxiv_Submission/11_Figure_Captions.tex <==
\newpage

\textbf{Figure captions}

\begin{itemize}
   \item \textbf{Figure 1}: \textbf{A weighted proportion of times a natural cubic spline representing a particular complementary football statistic (rows) was selected across different group penalties and tuning parameter selection approaches.}
   
   \item \textbf{Figure 2}: \textbf{Non-linear effects of complementary statistics on respective response categories, controlling for strength of schedule and homefield factor. Left: Effect of non-scoring turnovers forced by your defense on points scored by your offense. Right: Effect of per-play yardage allowed by your defense on yards gained by your offense.} These particular effect graphics were obtained for a Navy versus Army match-up at a neutral site. Changing the match-up would only affect the intercepts, hence there's no loss of generality in depicting the nature of the effect.
   
\end{itemize}

==> Arxiv_Submission/9_Tables.tex <==

\newpage


\begin{table}[H]
    \centering
    
 \begin{tabular}{rcc}
Team & Points Scored & Non-Scoring Turnovers Forced \\ & (Per Game) & (Per Possession) \\ \hline  
 \begin{tabular}{r} \\ Oregon \\ Louisiana Tech \\ Texas A\&M \\ Oklahoma State \\ Baylor \\ Clemson \\ Oklahoma \\ Alabama \\ West Virginia \\ Tennessee \\ Texas Tech \\ Georgia  \\ .... \\ South Florida \\ .... \\ Washington  \\ .... \\ \end{tabular} &
 \begin{tabular}{rrrr} Value & (Shift) & Rank & (Shift)\\ \hline 48.43 & ($\textcolor{red}{\Downarrow}$ 1.02) & 1 & ($\textcolor{blue}{0}$) \\ 47.12 & ($\textcolor{darkgreen}{\Uparrow}$ 0.19) & 2 & ($\textcolor{blue}{0}$) \\ 46.67 & ($\textcolor{darkgreen}{\Uparrow}$ 0.75) & 3 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 46.15 & ($\textcolor{darkgreen}{\Uparrow}$ 0.11) & 4 & ($\textcolor{red}{\Downarrow}$ 1) \\ 45.25 & ($\textcolor{darkgreen}{\Uparrow}$ 0.01) & 5 & ($\textcolor{blue}{0}$) \\ 41.02 & ($\textcolor{darkgreen}{\Uparrow}$ 0.08) & 6 & ($\textcolor{blue}{0}$) \\ 40.93 & ($\textcolor{darkgreen}{\Uparrow}$ 0.26) & 7 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 40.57 & ($\textcolor{red}{\Downarrow}$ 0.17) & 8 & ($\textcolor{red}{\Downarrow}$ 1) \\ 39.74 & ($\textcolor{red}{\Downarrow}$ 0.06) & 9 & ($\textcolor{blue}{0}$) \\ 39.69 & ($\textcolor{darkgreen}{\Uparrow}$ 0.58) & 10 & ($\textcolor{darkgreen}{\Uparrow}$ 2) \\ 39.44 & ($\textcolor{darkgreen}{\Uparrow}$ 1.22) & 11 & ($\textcolor{darkgreen}{\Uparrow}$ 4) \\ 38.98 & ($\textcolor{red}{\Downarrow}$ 0.19) & 12 & ($\textcolor{red}{\Downarrow}$ 1) \\ ... & ... \\21.99 & ($\textcolor{darkgreen}{\Uparrow}$ 1.16) & 87 & ($\textcolor{darkgreen}{\Uparrow}$ 6) \\ ... & ... \\23.72 & ($\textcolor{red}{\Downarrow}$ 1.02) & 80 & ($\textcolor{red}{\Downarrow}$ 5) \\ ... & ... \\ \end{tabular} & 
 \begin{tabular}{rr} \n Value & Rank \\ \hline 0.19 & 4 \\ 0.13 & 52 \\ 0.08 & 114 \\ 0.12 & 75 \\ 0.12 & 61 \\ 0.12 & 67 \\ 0.09 & 111 \\ 0.17 & 13 \\ 0.10 & 97 \\ 0.09 & 108 \\ 0.06 & 124 \\ 0.16 & 23 \\ ... & ... \\0.06 & 123 \\ ... & ... \\0.19 & 5 \\ ... & ... \\ \end{tabular}
\end{tabular}
    \caption{\textbf{Final 2012 season rankings (and ranking shifts) in points scored per game by team's offense, adjusted for defense's ability to turn the ball over to team's offense.}
    }
    \label{tab:RankShiftsOffense}
\end{table}
 
 
  \
 
 \
 
\begin{table}[H]
    \centering
 \begin{tabular}{rcc} 
 Team & Points Allowed & Non-Scoring Turnovers Committed \\ & (Per Game) & (Per Possession) \\ \hline  
 \begin{tabular}{r} \\ Alabama \\ Notre Dame \\ Florida \\ Michigan State \\ Stanford \\ Brigham Young \\ South Carolina \\ Florida State \\ Rutgers \\ Kansas State \\ Louisiana State \\ Texas Christian  \\ .... \\ Pittsburgh \\ .... \\ Illinois  \\ .... \\ \end{tabular} &
 \begin{tabular}{rrrr} Value & (Shift) & Rank & (Shift)\\ \hline  8.70 & ($\textcolor{red}{\Uparrow}$ 0.42) & 1 & ($\textcolor{blue}{0}$) \\ 11.85 & ($\textcolor{red}{\Uparrow}$ 0.42) & 2 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 11.88 & ($\textcolor{red}{\Uparrow}$ 0.80) & 3 & ($\textcolor{red}{\Downarrow}$ 1) \\ 14.03 & ($\textcolor{red}{\Uparrow}$ 0.46) & 4 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 14.05 & ($\textcolor{red}{\Uparrow}$ 0.88) & 5 & ($\textcolor{red}{\Downarrow}$ 1) \\ 14.26 & ($\textcolor{red}{\Uparrow}$ 0.10) & 6 & ($\textcolor{blue}{0}$) \\ 15.74 & ($\textcolor{darkgreen}{\Downarrow}$ 0.60) & 7 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 15.97 & ($\textcolor{darkgreen}{\Downarrow}$ 0.44) & 8 & ($\textcolor{darkgreen}{\Uparrow}$ 1) \\ 16.56 & ($\textcolor{darkgreen}{\Downarrow}$ 0.31) & 9 & ($\textcolor{darkgreen}{\Uparrow}$ 2) \\ 16.84 & ($\textcolor{red}{\Uparrow}$ 0.88) & 10 & ($\textcolor{red}{\Downarrow}$ 3) \\ 17.06 & ($\textcolor{red}{\Uparrow}$ 0.25) & 11 & ($\textcolor{red}{\Downarrow}$ 1) \\ 17.31 & ($\textcolor{darkgreen}{\Downarrow}$ 0.60) & 12 & ($\textcolor{darkgreen}{\Uparrow}$ 2) \\ ... & ... \\25.07 & ($\textcolor{red}{\Uparrow}$ 1.26) & 51 & ($\textcolor{red}{\Downarrow}$ 8) \\ ... & ... \\27.41 & ($\textcolor{darkgreen}{\Downarrow}$ 1.27) & 64 & ($\textcolor{darkgreen}{\Uparrow}$ 5) \\ ... & ... \\ \end{tabular} & 
 \begin{tabular}{rr} \n Value & Rank \\ \hline 0.09 & 21 \\ 0.10 & 32 \\ 0.09 & 19 \\ 0.09 & 14 \\ 0.10 & 29 \\ 0.13 & 70 \\ 0.13 & 77 \\ 0.15 & 92 \\ 0.13 & 69 \\ 0.08 & 9 \\ 0.10 & 33 \\ 0.16 & 104 \\ ... & ... \\0.06 & 2 \\ ... & ... \\0.20 & 124 \\ ... & ... \\ \end{tabular}
 \end{tabular}
    \caption{\textbf{Final 2012 season rankings (and ranking shifts) in points allowed per game by team's defense, adjusted for offense's ability to avoid turning the ball over to opposing offense.}
    }
    \label{tab:RankShiftsDefense}
\end{table}


 
 
 
\newpage



\begin{table}[H]
    \centering
 \begin{tabular}{rcc}
 & Binary Game Outcome & Score Differential \\
Adjustment &  (Won/Lost, AUROC)  & (MAE)  \\
\hline
\begin{tabular}{r}
\\
None \\
SOS+HF \\
SOS+HF \& Efficiency Cmpl. \\
SOS+HF \& Any Cmpl. \\
\end{tabular} &

\begin{tabular}{rr} 
Training & Test \\
\hline
0.790 (0.017) & 0.704 (0.028) \\
0.810 (0.017) & 0.715 (0.026) \\
 0.808 (0.016) & 0.717 (0.033) \\
 0.790 (0.019) & 0.707 (0.026) \\
\end{tabular} &

\begin{tabular}{rr} 
Training & Test \\
\hline
14.76 (0.57) & 17.39 (1.20) \\
13.78 (0.58) & 17.12 (1.18) \\
13.83 (0.57) & 17.13 (1.18) \\
14.58 (0.58) & 17.53 (0.93) \\
\end{tabular}

\end{tabular}
 \caption{\textbf{Predicting binary game outcomes (won/lost) via logistic regression, and numerical scoring differentials via linear regression, across 2009-2019 seasons by using variously adjusted points per game margin stats.} Training metric obtained from fitting the model to entire season, while test metric is obtained from using only first 9 weeks to predict the rest of the season.}
    
    \label{tab:PredictionEvaluationLinearMethods}
\end{table}














